Reward Engineering for Software Tasks: A Survey of Reinforcement Learning Approaches

Reinforcement learning is increasingly used for code-centric software engineering tasks, including code generation, understanding, repair, testing, and optimization, especially with the rise of large language models and autonomous agents. A core challenge in these settings is reward design. Unlike standard RL domains with clear scalar objectives, software tasks involve competing goals such as correctness, security, efficiency, and readability, which are difficult to capture with a single reward. As a result, RL-for-SE systems rely on heterogeneous signals, including compilation results, unit tests, coverage metrics, retrieval scores, and learned preferences. Yet this work remains scattered across tasks and communities. This survey provides the first systematic review of reward engineering for RL in software tasks. We organize prior work by reward source, granularity, and aggregation. We then distill the findings into practical guidance, including a decision matrix, a design guide, and a reward engineering reporting standard for future RL-for-SE systems.

==> latex/003-codetasks/4-codesecurity/2-vulnerabilityrepair.tex <==
% \subsubsection{Vulnerability Repair}

% Vulnerability repair often admits multiple valid patches and may lack reliable tests, making \textit{execution}-based rewards sparse or impractical. PairCode~\cite{islam2024code} fine-tunes a causal LLM with PPO using a reference-based \textit{similarity} reward, combining a syntactic CodeBLEU score and a semantic BERTScore against the ground-truth patch, $R = R_{\text{CodeB}} + R_{\text{BERT}}$, providing execution-free guidance that biases the model toward surface- and embedding-level similarity rather than behavioral correctness. SecRepair~\cite{islam2024llm} applies RL at the commit-comment generation stage, optimizing BERTScore-based similarity to ensure generated descriptions preserve the semantics of the ground-truth comment, targeting documentation quality rather than patch execution. Vul-R2~\cite{wen2025vul} integrates a verifiable critic with reference shaping, assigning reward
% \begin{equation}
% \small
% R = 
% \begin{cases}
% -2, & \text{if the patch is judged as incorrect},\\
% 1 + \mathrm{Sim}(o,\mathrm{GT}), & \text{otherwise},
% \end{cases}
% \end{equation}
% where $\mathrm{Sim}\in[0,1]$ measures similarity to the human patch, combining \textit{preference}-based verification with \textit{similarity}-based shaping. Overall, RL in vulnerability repair emphasizes dense similarity and model-judged preference rewards, reflecting the challenges of sparse execution feedback and multiple valid solutions.

\subsubsection{Vulnerability Repair}

Vulnerability repair often admits multiple valid patches and may lack reliable tests, making \textit{execution}-based rewards sparse. PairCode~\cite{islam2024code} fine-tunes a causal LLM with PPO using a reference-based \textit{similarity} reward that sums CodeBLEU and BERTScore against the ground-truth patch, $R = R_{\text{CodeB}} + R_{\text{BERT}}$, providing execution-free guidance but biasing toward surface/semantic similarity rather than behavior. SecRepair~\cite{islam2024llm} instead applies RL to commit-comment generation, optimizing BERTScore similarity to preserve the semantics of the ground-truth comment. Vul-R2~\cite{wen2025vul} combines a verifiable critic with reference shaping:
\begin{equation}
\small
R =
\begin{cases}
-2, & \text{if the patch is judged incorrect},\\
1 + \mathrm{Sim}(o,\mathrm{GT}), & \text{otherwise},
\end{cases}
\end{equation}
where $\mathrm{Sim}\in[0,1]$ measures similarity to the human patch. Overall, RL for vulnerability repair favors dense similarity and model-judged \textit{preference} rewards due to sparse execution feedback and patch multiplicity.








% Vulnerability repair often admits multiple correct patches and may lack reliable tests, making \textit{Execution} rewards sparse or costly. As a result, recent RL approaches frequently rely on dense \textit{Similarity} shaping against reference patches, sometimes combined with model-judged correctness signals.

% \paragraph{PairCode.}
% PairCode ~\cite{islam2024code} fine-tunes a causal LLM with PPO using a reference-based \textit{Similarity} reward.
% The terminal reward is the sum of a syntactic score based on CodeBLEU and a semantic score based on BERTScore,
% both computed against the ground-truth repair:
% $R = R_{\text{CodeB}} + R_{\text{BERT}}$.
% This provides execution-free training feedback that biases the policy toward patches closer to human repairs in
% surface structure and embedding-level similarity, rather than behavioral correctness via test execution.


% \paragraph{SecRepair.}
% SecRepair~\cite{islam2024llm} applies RL only in the final code/commit-comment generation stage (not in patch generation).
% Using PPO, it fine-tunes a description-to-comment model with a reference-based \textit{Similarity} reward based on BERTScore,
% encouraging the generated short comment to preserve the semantics of the ground-truth commit comment.
% Accordingly, the RL objective targets the communication/documentation quality of repairs rather than patch correctness via execution.


% \paragraph{Vul-R2.}
% Vul-R2~\cite{wen2025vul} trains with RLVR using a verifiable reward that combines an LLM-based verifier with reference shaping.
% A critic LLM outputs a binary correctness judgment; if incorrect, the answer reward is set to a negative value (e.g., $-2$),
% otherwise it becomes $1+\mathrm{Sim}(o,\mathrm{GT})$, where $\mathrm{Sim}\in[0,1]$ measures similarity to the human ground-truth patch
% (character-level matching in the hard stage).
% In our taxonomy, this mixes \textit{Preference/Verifier} (critic judgment) with \textit{Similarity} (reference matching).



==> latex/003-codetasks/5-codetesting/2-fuzzing.tex <==
\subsubsection{Fuzzing}

% Reinforcement learning for fuzzing primarily leverages \textit{Execution}-derived feedback, combining coverage signals to guide exploration and oracle-based execution outcomes to bias input generation toward valid or security-relevant behaviors. REINAM~\cite{wu2019reinam} uses a binary reward based on program acceptance, assigning $1$ if the generated input is accepted and $0$ otherwise, representing a straightforward \textit{execution} signal. RLF~\cite{su2022effectively} combines an \textit{execution} vulnerability reward, $R_{\text{bugs}}$, with a block-level coverage reward, $R_{\text{cov}}$, via
% \begin{equation}
% \small
% R_{\text{mix}} = \alpha R_{\text{bugs}} + (1-\alpha) R_{\text{cov}},
% \end{equation}
% balancing vulnerability discovery with exploratory coverage. CovRL-Fuzz~\cite{eom2024fuzzing} introduces a TF--IDF-inspired coverage reward that upweights rarely covered code regions and applies explicit penalties for invalid inputs, ensuring that coverage optimization is conditioned on syntactically and semantically valid test cases. 
Fuzzing generates large volumes of (often mutated) inputs to exercise a program and expose crashes or vulnerabilities. RL for fuzzing mainly uses \textit{execution}-derived feedback, combining coverage signals for exploration with oracle-based outcomes to steer generation toward valid or vulnerability-triggering inputs. REINAM~\cite{wu2019reinam} uses a binary \textit{execution} reward ($1$ if the input is accepted, $0$ otherwise). 
% RLF~\cite{su2022effectively} mixes a vulnerability reward $R_{\text{bugs}}$ with block-level coverage $R_{\text{cov}}$ via $R_{\text{mix}}=\alpha R_{\text{bugs}}+(1-\alpha)R_{\text{cov}}$. 
RLF~\cite{su2022effectively} combines an \textit{execution} vulnerability reward, $R_{\text{bugs}}$, with a block-level coverage reward, $R_{\text{cov}}$, via
\begin{equation}
\small
R_{\text{mix}} = \alpha R_{\text{bugs}} + (1-\alpha) R_{\text{cov}},
\end{equation}
balancing vulnerability discovery with exploratory coverage.
CovRL-Fuzz~\cite{eom2024fuzzing} upweights rarely covered regions with a TF--IDF-style coverage reward and penalizes invalid inputs, conditioning coverage gains on valid test cases.
Overall, RL-guided fuzzing demonstrates how execution and coverage signals can be effectively combined to maximize both exploration and vulnerability detection in testing.

% RL-guided fuzzing typically relies on \textit{execution-derived} feedback: (i) \textit{Coverage} signals to drive exploration toward new program behaviors, and (ii) \textit{Execution} oracles (e.g., acceptance/rejection or vulnerability triggers) to bias search toward valid or security-relevant inputs.

% \paragraph{REINAM.}
% REINAM~\cite{wu2019reinam} treats the target program as a black-box oracle and assigns reward based on whether the fully constructed input is \emph{accepted} (1) or \emph{rejected} (0). 
% Under our taxonomy, this is an \textit{Execution} reward, since the signal is obtained by running/consulting the program to validate the generated input.

% \paragraph{RLF.}
% RLF~\cite{su2022effectively} uses an \textit{Execution} reward $R_{\text{bugs}}$ that is $1$ if its test-oracle detector identifies any triggered vulnerability during fuzzing, and $0$ otherwise. 
% It also uses a block-\textit{Coverage} reward $R_{\text{cov}}$ (computed from basic-block coverage, averaged across function groups), and combines them via
% $R_{\text{mix}}=\alpha R_{\text{bugs}}+(1-\alpha)R_{\text{cov}}$ to balance vulnerability finding and exploration.


% \paragraph{CovRL.}
% CovRL-Fuzz~\cite{eom2024fuzzing} proposes a TF--IDF-style \textit{Coverage} reward (Coverage-Weighted Rewarding, CWR) that upweights \emph{less common} coverage points via an IDF-like weight map and rewards the weighted sum of a \emph{unique} coverage map, explicitly encouraging exploration of under-covered code.
% \textit{Execution} outcomes also act as a validity signal: invalid inputs receive explicit penalties (e.g., $-1.0$ for syntax errors and $-0.5$ for semantic errors), and the coverage-weighted reward is computed only when the generated test case is free of syntax/semantic problems.

